LoopTree: Exploring the Fused-layer Dataflow Accelerator Design Space

Latency and energy consumption are key metrics in the performance of deep neural network (DNN) accelerators. A significant factor contributing to latency and energy is data transfers. One method to reduce transfers or data is reusing data when multiple operations use the same data. Fused-layer accelerators reuse data across operations in different layers by retaining intermediate data in on-chip buffers, which has been shown to reduce energy consumption and latency. Moreover, the intermediate data is often tiled (i.e., broken into chunks) to reduce the on-chip buffer capacity required to reuse the data. Because on-chip buffer capacity is frequently more limited than computation units, fused-layer dataflow accelerators may also recompute certain parts of the intermediate data instead of retaining them in a buffer. Achieving efficient trade-offs between on-chip buffer capacity, off-chip transfers, and recomputation requires systematic exploration of the fused-layer dataflow design space. However, prior work only explored a subset of the design space, and more efficient designs are left unexplored. In this work, we propose (1) a more extensive design space that has more choices in terms of tiling, data retention, recomputation and, importantly, allows us to explore them in combination, (2) a taxonomy to systematically specify designs, and (3) a model, LoopTree, to evaluate the latency, energy consumption, buffer capacity requirements, and off-chip transfers of designs in this design space. We validate our model against a representative set of prior architectures, achieving a worst-case 4% error. Finally, we present case studies that show how exploring this larger space results in more efficient designs (e.g., up to a 10$\times$ buffer capacity reduction to achieve the same off-chip transfers).

==> figures/background/channel_row.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{images/background/channel_row.pdf}
    \caption{Tiles of iterations 0-3 in a dataflow with intermediate-channel tiling followed by row tiling. \figtakeaway this dataflow has smaller tiles (compare Fmap2 tiles here and Fig.~\ref{fig:background:tiling}(a)) and always requires a smaller buffer capacity compared to intermediate-channel tiling.}
    \label{fig:background:channel_row}
\end{figure}

==> figures/background/channel_tiling.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{images/background/tiling.pdf}
    \caption{\textbf{(a)} Tiles (darker shade) of Fmap1, Fmap2, and Fmap3 in iterations 0 and 1 in an intermediate-channel ($C2$ rank) tiling. Computing one Fmap2 channel requires all Fmap1 channels as inputs. Similarly, one Fmap2 channel is used to compute all Fmap3 channels. \textbf{(b)} Tiles (darker shade) of Fmap1, Fmap2, and Fmap3 in iterations 0 and 1 in a output row ($P2$ rank) tiling. The Fmap2 tiles of the intermediate-channel tiling (a) do not overlap across iterations 0 and 1 but tiles in row tiling (b) do, which results in no recompute choices (a) but choices for (b). \figtakeaway{Only some tiling choices lead to recompute choices}.}
    \label{fig:background:tiling}
\end{figure}

==> figures/background/per_layer_reuse_recompute.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.475\textwidth]{images/background/per_layer_reuse_recompute.pdf}
    \caption{Comparing row tiling dataflow for three 1D convolution layers that recomputes all intermediate fmaps (top) and mixes retain and recompute (bottom). See points (1), (2), and (3). \figtakeaway{Mixing retain-recompute choices for different fmaps can reduce the amount of recomputation}.}
    \label{fig:background:per_layer_reuse_recompute}
\end{figure}

==> figures/background/uneven.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/background/uneven.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

==> figures/case_study/buffer_size.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.425\textwidth]{images/case_study/buffer_size.png}
    \caption{Impact of flexible tiling choices for different sets of fused layers. Figure shows the size of on-chip buffer to capture all reuse within fused layers for $C2$-tiling and $P2,Q2$-tiling. Layers 1-3 have kernels with width 3 and 64, 128, 256, and 512 channels respectively. $P2,Q2$-tiling requires smaller buffers for early layers with fewer channels and vice versa. Flexible-tiling (this work) requires the smallest buffer size.}
    \label{fig:case_study:buffer_size}
\end{figure}

==> figures/case_study/conv_all.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{images/case_study/conv_all.pdf}
    \caption{Pareto-optimal dataflow choices for fusing two 2D convolution layers. Subplot titles denote width (height is the same) and channels. The y-axis is off-chip transfers in Mwords (\ie, $10^6$ words). The x-axis is the buffer capacity in Kwords. Color denotes the amount of recomputation (blue is low, purple is high). Shapes denote dataflows as follows. Square: $C2,P2$-tiling, diamond: $P2,Q2,C2$-tiling, plus: $P2,Q2$-tiling, triangle: $C2$-tiling. No single dataflow choice is optimal in all scenarios. Dataflows introduced in this paper (square and diamond) make up for significant portion of the Pareto-optimal choices.}
    \label{fig:case_study:conv_all}
\end{figure}

==> figures/case_study/cpq.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.425\textwidth]{images/case_study/cpq.png}
    \caption{Impact of exploring additional tiling. Required buffer size (bars) and off-chip transfers (line) of input and output fmaps are shown for $C2$-tiling and $C2,P2,Q2$-tiling. Off-chip transfers are independent of tiling. Tiling in certain dimensions does not increase off-chip transfers but reduces buffer size.}
    \label{fig:case_study:cpq}
\end{figure}

==> figures/case_study/evaluating_further_tiling_c.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.475\textwidth]{images/case_study/mbconv.c+cpq.pdf}
    \caption{Buffer capacity and recomputation tradeoff Pareto curve for $C3$ tiling and $C3,P3,Q3$ tiling. \figtakeaway{$C3,P3,Q3$ tiling is more efficient than $C3$ tiling. Furthermore, $C3,P3,Q3$ tiling allows trading off capacity with recomputation, while $C3$ tiling does not because there is no intermediate fmap reuse.}}
    \label{fig:case_study:evaluating_further_tiling_c}
\end{figure}

==> figures/case_study/evaluating_further_tiling_p.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.475\textwidth]{images/case_study/mbconv.pq+pcq.pdf}
    \caption{Buffer capacity and recomputation tradeoff Pareto curve for $P3,Q3$ tiling and $P3,C3,Q3$ tiling. \figtakeaway{$P3,C3,Q3$ tiling is more efficient than $P3,Q3$ when the number of channels ($C3$) is high.}}
    \label{fig:case_study:evaluating_further_tiling_p}
\end{figure}

==> figures/case_study/fc.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{images/case_study/fc.pdf}
    \caption{Buffer capacity required to achieve minimum algorithmic transfers for $D2$-tiling dataflow and $M$-tiling dataflow when processing fused FC-FC workloads of various shapes. The baseline has rank sizes $M=D1=D2=D3=512$. When not specified, a rank has the same size as in the baseline. The tiling that leads to lower buffer capacity depends on the workload shape.}
    \label{fig:case_study:fc}
\end{figure}

==> figures/case_study/per_layer_recompute.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.425\textwidth]{images/case_study/per_layer_recompute.png}
    \caption{Impact of per-layer retain-recompute choices. The number of operations (y-axis) against the required buffer size (x-axis) are shown when recomputing both Conv1+Conv2 (Pareto in prior work~\cite{defines}) and only Conv1 (Pareto in this work). Choosing per-layer reuse/recompute choices can limit the compounding effect of recomputation.}
    \label{fig:case_study:per_layer}
\end{figure}

==> figures/case_study/per_tensor_breakdown.tex <==
\begin{figure}
    \centering

    \caption{TODO}
    \label{fig:case_study:per_tensor_breakdown}
\end{figure}

==> figures/case_study/pqc.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.425\textwidth]{images/case_study/pqc.png}
    \caption{Exploring the interaction of tiling and reuse/recompute choices. The number of operations (y-axis) and buffer size (x-axis) are shown for $P2,Q2$-tiling with no-retain and $P2,Q2,C2$-tiling with $C2$-retain. Exploring tiling in conjunction with reuse/recompute choices allows us to find designs with less buffer space for the same recomputation.}
    \label{fig:case_study:pqc}
\end{figure}

==> figures/case_study/pwise_dwise_pwise_breakdown.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.475\textwidth]{images/case_study/pwise+dwise+pwise.breakdown.pdf}
    \caption{Breakdown of buffer capacity usage by tensors of a single tiling chosen from Fig.~\ref{fig:case_study:pwise+dwise+pwise} for different fusion set shapes at different amounts of recomputation. The impact of recomputation on buffer capacity required by different tensors depends on the tiling.}
    \label{fig:case_study:pwise_dwise_pwise_breakdown}
\end{figure}

==> figures/design_space/inter_layer_tiling.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{images/design_space/inter_layer_tiling.pdf}
    \caption{Examples of inter-layer tiling. (a) The result of partitioning $P2$ (rank $P$ of layer Conv2) in a fusion set of two 1D convolution layers (filters not shown). Specifying tiling for Conv2 is enough to determine the tiling of all fmaps and operations of Conv1 (see Section~\ref{sec:model:analyzing_tile_shapes}). (b) Tiling $P2$ and $Q2$ in a fusion set of two 2D convolution layers. In both figures, the first two tiles are shown (first tile is dashed and second tile solid).}
    \label{fig:design_space:tiling}
\end{figure}

==> figures/design_space/intra_layer_tiling.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.46\textwidth]{images/design_space/intra_layer_tiling.pdf}
    \caption{Intra-layer tiling can be performed independently for each layer. In this example, we: (a) intra-layer tile rank $P1$ within each Conv1 tile, and (b) intra-layer tile rank $R2$ within each Conv2 tile.}
    \label{fig:design_space:intra_layer_tiling}
\end{figure}

==> figures/design_space/iterations.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.3\textwidth]{images/design_space/iterations.pdf}
    \caption{Iterations in a $P2,Q2$ tiling and the corresponding rank iterations. We denote iterations across a rank with lowercase variables. Within the iterations row, we used $P2$ and $Q2$ to denote the shape of the corresponding ranks.}
    \label{fig:design_space:iterations}
\end{figure}

==> figures/design_space/reuse_row.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.3\textwidth]{images/design_space/reuse_row.pdf}
    \caption{Tiles of Conv1 and Conv2 when retaining reused Fmap2 across iterations of $P2$. Compared to Fig.~\ref{fig:design_space:tiling}(a), Conv1 Tile1 is smaller, indicating a smaller amount of operations to process.}
    \label{fig:design_space:reuse_row}
\end{figure}

==> sections/10.conflict_of_interest.tex <==
\section*{Conflicts of Interest}
We would like to declare conflicts of interest with reviewers affiliated with MIT, Google, and NVIDIA, due to the authors' affiliations.

==> tables/case_study/mapspace_size.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
    Fusion set & \multicolumn{2}{c}{Mapspace size reduction (orders of magnitude)}  \\
               & Retain choice & Tile shape \\
\hline
    conv+conv & 3 & 1 \\
    conv+conv+conv & 3 & 1 \\
    pwise+dwise+pwise & 3 & 2 \\
    fc+fc & 3 & 2 \\
\bottomrule
\end{tabular}
\caption{Reduction in mapspace size when using algorithmic minimum off-chip transfers heuristic to prune retain choices and tile shape.}
\label{tab:case_study:pruning}
\end{table}

==> tables/heuristic/retain.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{@{} lcccc @{}}
    \toprule
    \makecell[l]{Tiled ranks \\ (schedule: top to bottom)} & \multicolumn{4}{c}{Reuse} \\
     & \makecell[c]{Input \\ fmap} & \makecell[c]{Output \\ fmap} & \makecell[c]{Intermediate \\ fmap} & Filters \\
     \hline
     Output rows ($P2$) & Conv. & None & Conv. & Full \\
     Intermediate channel ($C2$) & Full & Full & None & None \\
     \bottomrule
    \end{tabular}
    \caption{Reuse across each rank iteration in $P2,C2$ tiling (listed top to bottom in table). If filters are not retained across output rows ($P2$), they will be refetched from off-chip. Thus, filters need to be retained across $P2$ iterations. Input fmap is reused in both $P2$ and $C2$, thus we specify input fmap to be retained across $P2$ in order to retain across both.}
    \label{tab:heuristic:retain}
\end{table}

==> tables/introduction/comparison.tex <==
\begin{table*}
\caption{Comparison of design space in prior works and the larger design space in this work. *Ranks: also called dimensions in other works (\eg, channels, rows, columns). Prior works have significant limitations in their design space.}
\label{tab:introduction:comparison}
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
    Framework & \makecell{Tiled ranks*} & \makecell{Retain-recompute} & \makecell{Per-layer retain-recompute} & Supported Workload \\
\hline
    TANGRAM~\cite{tangram} & \textcolor{BrickRed}{Channel} & \textcolor{BrickRed}{No} & \textcolor{BrickRed}{No} & \textcolor{OliveGreen}{Any} \\
    DeFiNES~\cite{defines} & \textcolor{BrickRed}{Row \& column} & \textcolor{OliveGreen}{Yes} & \textcolor{BrickRed}{No} & \textcolor{BrickRed}{CNN} \\
    Stream~\cite{stream} & N/A & \textcolor{BrickRed}{No} & \textcolor{BrickRed}{No} & \textcolor{OliveGreen}{Any} \\
    ConvFusion~\cite{convfusion} & \textcolor{BrickRed}{Row \& column} & \textcolor{OliveGreen}{Yes} & \textcolor{BrickRed}{No} & \textcolor{BrickRed}{CNN} \\
    Optimus~\cite{optimus} & \textcolor{BrickRed}{Row \& column} & \textcolor{OliveGreen}{Yes} & \textcolor{BrickRed}{No} & \textcolor{BrickRed}{CNN} \\
    SET\cite{set} & \textcolor{BrickRed}{Batch} & \textcolor{BrickRed}{No} & \textcolor{BrickRed}{No} & \textcolor{OliveGreen}{Any} \\
    This work & \textcolor{OliveGreen}{Any} & \textcolor{OliveGreen}{Yes} & \textcolor{OliveGreen}{Yes} & \textcolor{OliveGreen}{Any} \\
\bottomrule
\end{tabular}

\end{table*}
